Unveiling Low-Frequency Eclipses in Spider MSPs using wideband GMRT Observations

Eclipses of radio emission have been reported for ~ 58 spider millisecond pulsars (MSP), of which only around 19% have been extensively studied. Such studies at low frequencies are crucial for probing the properties of the eclipse medium, as eclipses are more prominent at such frequencies. This study investigates eclipses in 10 MSPs in compact orbit using wide-bandwidth observations with the upgraded Giant Metrewave Radio Telescope. We report the first evidence of eclipsing for PSR J2234+0944 and J2214+3000 in one epoch, while no evidence of eclipsing was observed in the subsequent two epochs, indicating temporal evolution of the eclipse cutoff frequency in these systems. Constraints on the eclipse cutoff frequency were obtained for PSR J1555-2908, J1810+1744, and J2051-0827. Moreover, for the first time, we detected an eclipse at a non-standard orbital phase (~ 0.5) for PSR J1810+1744, with a duration longer than the eclipse observed at superior conjunction. No eclipses were detected for PSR J0751+1807, J1738+0333, and J1807-2459A at 300-500 MHz and 550-750 MHz, for which we discuss the possible reasons. We calculated the mass loss rates of the companions for PSR J1555-2908 and PSR J1810+1744, and found that these rates are insufficient to ablate the companion stars. We cataloged the $\dot{E}/a^2$, mass function, roche lobe filling factor, and inclination angle for compact MSP binaries with low-mass companions and found that higher spin-down flux does not guarantee eclipses. Our analysis, supported by the Kolmogorov-Smirnov statistic, reveals that eclipsing black widow binaries generally exhibit a higher mass function compared to non-eclipsing black widow binaries, as reported by previous studies for a limited sample of black widow MSPs.

==> table1.tex <==
\begin{table*}[!htb]
\begin{center}
\caption{Summary of the observations}
\label{tab:Table1}
\vspace{0.3cm}
\label{discovery}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
Pulsar name     & P$^{a}$ & DM$^{b}$ & $P_{b}^{c}$ &Freq & OP$^{d}$ & Date & $\nu_{c}$ & $N_{e}^{e}$ & $R_{E}^{g}$& $M_{c}^{h}$\\
     & (ms)& ($pc~cm^{-3}$)& & (MHz) &  &  & (MHz) & $(10^{16}cm^{-2})$  &(cm) & ($\mathrm{M}_\odot/year$)\\
\hline
 
J0751+1807 & 3.47 &30.24& 6.31 & B34 &  0.16-0.31& 03 December 2022 &-   & - & -&-\\

\hline
J1431--4715 & 2.01 &59.35& 10.79 & B34 & 0.20-0.31 & 25 November 2022  & -  &-  & -&-\\
  &   & &  & B3 & 0.22-0.36 & 04 November 2023  & -  & - &- &-\\
\hline 
J1555--2908& 1.78 &75.91&   & B34  & 0.20-0.38 & 29 June 2020  &  $>$ 740&  7.3  &- &-\\
 &  &&   & B45  &  0.13-0.55 &  04 July 2020 & $>$ 740 &  11.7 &6.6 $\times 10^{10}$& 8.2 $\times 10^{-13}$\\
\hline  
J1738+0333& 5.85&33.77&  8.51  & B34 &  0.08-0.27& 9 January 2023 & - &  -& -&-\\
\hline
J1807--2459A&3.05&134.00&  1.70   & B32 &  0.47-1.19& 03 June 2020 & - &  & -&-\\
 & & &      & B3  &  0.01-0.73 & 11 June 2020$_{1}$  & - &  - & -&-\\
  & & &      & B3  &  0.80-1.42 & 11 June 2020$_{2}$  & - &  - & -&-\\
  & & &      & B45  & 0.89-1.57 & 27 June 2020  & $<$ 550 &  -  & -&-\\
\hline
J1810+1744  & 1.66 & 39.70 & 3.60 &  B45 &  0.12-0.82 & 26 June 2020$_{1}$&  $>$ 740  & 7.6  &1.5$\times 10^{11}$& 8.7$\times 10^{-13}$\\
   & & & &  B45 & 0.94-1.64& 26 June 2020$_{2}$&  $>$ 740 & 4.3 & 1.5$\times 10^{11}$ & 6.5$\times 10^{-13}$\\
\hline
J2051--0827&4.50&20.73& 2.37& B45 &  0.12-0.75 & 19 June $2020_{1}$&  $<$ 640   & 10.9 &  &\\
&&& &  &  0.85-1.82 & 19 June $2020_{2}$& $<$ 640  & 14.4  &- &-\\
 & & &  &   & 0.92-1.48  & 19 June $2020_{3}$& $<$ 640  & 16.9 & - &-\\
\hline
 J2214+3000  &3.11&22.54&  9.99 &  B34& 0.20-0.26 & 11 November 2022& - &  & & \\
    & & &    &  B34& 0.19-0.33 & 30 October 2023& - & - & - &- \\
    & & &    &  B34& 0.18-0.32 & 06 November 2023& -& -  & - & -\\
\hline
J2215+5135   &2.61&69.20&   4.14  & B34 &0.07-0.43 & 11 November 2022 &- &  -&- &-\\
    & & &      &  B3 & 0.03-0.37 & 29 October 2023 &- & - &- &-\\
& & &      &  B3 & 0.19-0.31  & 04 November 2023 & - & - &- &-\\
\hline
J2234+0944   &3.62&17.83&  10.07     &B34 & 0.22-0.28 & 11 November 2022  & - & - & -&-\\
 & & &      & B34 & 0.20-0.34 & 29 October 2023& -  & - &- &-\\
    & & &      & B34 & 0.18-0.32 & 05 November 2023& - & - &- &-\\
\hline


\end{tabular}
\end{center}
$^{a}$: Spin period of the pulsar; $^{b}$: Dispersion measure; $^{c}$: Orbital period of the pulsar; $^{d}$: Orbital phase covered; $^{e}$: The maximum electron column density in the eclipse medium; $^{g}$: Eclipse radius; $^{h}$: Mass loss rate of the companion.

\vspace{1cm}
\end{table*}

==> table3.tex <==
\begin{table*}[hbt!][p]
\begin{center}
\caption{Table listing the $\dot{E}/a^{2}$, orbital inclination angle and Roche lobe filling factor (RLFF) values for the spider MSPs.}
\label{tab:Table3}
\vspace{0.3cm}
\label{table2}
\begin{longtable}[c]{|c|c|c|c|c|c|}
\hline
Pulsar name  & $\dot{E}/a^{2}$ & Inclination& RLFF & Mass function& References\\
& ($\times 10^{35} erg/s $\(R_\odot\)$^{2}$) & (degrees) & & &\\
\hline
J0023+0923 & 0.09&  58 $\pm$ 14 &0.3 &0.000002 &\\
J0024--7204I & & & &0.000001&\\
J0024--7204J & & & &0.000005&\\
\bf{J0024--7204O} &0.39  & & &0.000005&\\
J0024--7204P & 2.96& & &0.000003&\\
\bf{J0024--7204R} &2.22 & & &0.000009&\\
J0024--7204U & 0.05& & & 0.000853&\\
J0024--7204V & & & &0.009744&\\
J0024--7204W & & & &0.000876&\\
J0024--7204Y & & & &0.001178&\\
J0024--7204ac & & & &0.000000&\\
J0024--7204ad & & & &0.003297&\\
\bf{J0251+2606} & 0.06& & &0.000007&\\
J0312--0921 & 0.14& & &0.000000&\\
J0610--2100 &0.01 &54  $<$ i $<$ 89 &  0.72 $< f_{RL} <$ 0.94&0.000005&\\
J0636+5128 & 0.09& 24,40& 0.83,0.97&0.000000&\\
J0751+1807 & 0.03& & &0.000967&\\
J0952--0607 &0.16 & 59.8& 0.79&0.000004&\\
J1012+5307 & 0.003& & &0.000578&\\
J1023+0038 & 0.19& & &0.001107&\\
\bf{J1036--4353} & & & &0.004707&\\
J1036--8317 & & & &0.001239&\\
\bf{J1048+2339} & 0.02& & &0.010000&\\
\bf{J1124--3653} & 0.05&  44& 0.84&0.000011&\\
\bf{J1221--0633} &0.04 & & &0.000001&\\
\bf{J1227--4853} &0.18 &77 & 0.83&0.003870&\\
\bf{J1301+0833} & 0.15& 52 &0.57 &0.000007&\\
\bf{J1302--3258} & 0.002& & &0.001394&\\
\bf{J1311--3430} & 0.8& 60&0.99 &0.000000&\\
\bf{J1317--0157} & 0.09& & &0.000003&\\
J1326--4728B & & & &0.000001&\\
J1342+2822A & & & &0.000001&\\
\bf{J1431--4715} & 0.07&53-83 &0.64--0.76 &0.000883&\\
J1446--4701 & 0.08& & &0.000004&\\
\bf{J1513--2550} &0.38 & & &0.000002&\\
\bf{J1518+0204C} & 0.73& & &0.000027&\\
J1518+0204G & 0.18& & &0.000004&\\
J1526--2744 &0.03 & & &0.000294&\\
\bf{J1544+4937} & 0.07& & &0.000003&\\
\bf{J1555--2908} & 0.90& $>$ 75& 0.98&0.000068&\\
J1602--1009 &0.04 & & &0.000003&\\
\bf{J1622--0315} &0.03&$<$ 83.4 & &0.000433&\\
J1627+3219 & 0.09& & &0.000006&\\
\bf{J1628--3205} & 0.04&$>$ 55 & &0.001681&\\
J1630+3550 & 0.05& & &0.000001&\\
J1641+3627D & & & &0.002421&\\
\bf{J1641+3627E} &0.35 & & &0.000004&\\
\bf{J1641+8049} & 0.00004& 57&  $>$ 0.95&0.000034&\\
J1653--0158 & 0.26& & &0.000000&\\
\bf{J1701--3006B} & & & &0.000830&\\
J1701--3006C & & & &0.000167&\\
\bf{J1701--3006E} &1.78 & & &0.000015&\\
J1701--3006F & 2.56& & &0.000005&\\
J1701--3006G & & & &0.000427&\\
\bf{J1717+4308A} & 0.26& & &0.001687&\\
J1719--1438 & 0.01& & &0.000000&\\
J1720--0533 & 0.05& & &0.000013&\\
\bf{J1723--2837} & 0.03&30--41 & &0.005221&\\
J1727--2951 & 0.0007& & &0.000001&\\
\bf{J1731--1847} & 0.15& & &0.000019&\\
\bf{J1737-0314D} & & & &&\\
\bf{J1737-0314E} & & & &&\\
J1737--0314A & 1.50& & &0.000002&\\
J1738+0333 & 0.007& & &0.000346&\\
J1745+1017 & 0.003& & &0.000001&\\
\bf{J1745--23} & & & &0.000010&\\
J1748--2021D &0.02 & & &0.000822&\\
J1748--2446A & & & &0.000322&\\
J1748--2446M & & & &0.001158&\\
J1748--2446N & & & &0.030660&\\
J1748--2446O & & & &0.000022&\\
J1748--2446P & & & &0.016807&\\
J1748--2446V & & & &0.000772&\\
J1748--2446ab & & & &0.000322&\\
J1748--2446ae & & & &0.000002&\\
J1748--2446ai & & & &0.032863&\\
J1748--2446am & & & &0.001383&\\
J1753--2819 & & & &0.000066&\\
J1757--5322 &0.001 & & &0.047464&\\
\bf{J1803--6707} & 0.01& & &0.008882&\\
J1805+0615 &0.16 & & &0.000006&\\
J1807--2459A & & & &0.000000&\\
\bf{J1810+1744} & 0.21& & &0.000041&\\
\bf{J1816+4510} & 0.08& & &0.001740&\\
J1824--2452G & & & &0.000000&\\
J1824--2452H & & & &0.002113&\\
J1824--2452I & & & &0.002286&\\
J1824--2452J & & & &0.000002&\\
J1824--2452L & & & &0.000004&\\
J1824--2452M & 0.12& & &0.000001&\\
J1824--2452N &0.62 & & &0.000003&\\
J1833--3840 & 0.05& & &0.000000&\\
J1836--2354A & 0.008& & &0.000003&\\
J1850+0242 &0.04 & & &0.000184&\\
J1905+0154A & & & &0.000332&\\
J1906+0055 &0.004 & & &0.000705 &\\
J1908+2105 & 0.17& & &0.000080&\\
J1910--5959A & & & & 0.002688 &\\
J1911+0101A & & & &0.000003&\\
J1928+1245 & 0.14& & &0.000000&\\
J1946--5403 & 0.05& & &0.000005&\\
J1953+1844 & 0.34& & &0.000000&\\
J1953+1846A & & & &0.000016&\\
\bf{J1957+2516} & 0.04& & &0.000431&\\
\bf{J1959+2048} & 0.24& & &0.000005&\\
J2006+0148 & 0.009& & &0.001514&\\
J2017--1614 &0.07 & & &0.000009&\\
\bf{J2039--5617} & 0.08&61 $<$ i $<$ 78 & &0.002159&\\
J2047+1053 & 0.06& & &0.000023&\\
\bf{J2051--0827} & 0.05& & &0.000010&\\
\bf{J2052+1219} & 0.25& & &0.000019&\\
\bf{J2055+1545} & 0.12& & &0.005747&\\
J2055+3829 & 0.02& & &0.000006&\\
\bf{J2115+5448} &1.04 & & &0.000005&\\
J2129--0429 & & & &0.016848&\\
J2140--2310A & & & &0.000460&\\
J2214+3000 &0.02 & & &0.000001&\\
\bf{J2215+5135} &0.30 & 66& 0.99&0.003702&\\
\bf{J2234+0944} & 0.02& & &0.000002&\\
\bf{J2241--5236} & 0.14& & &0.000001&\\
\bf{J2256--1024} & 0.12& 68 $\pm$ 11& 0.40 $\pm$ 0.20&0.000014&\\
J2322--2650 & 0.001& & &0.000000&\\
J2339--0533 & 0.07& & &0.006589&\\
\hline



%\end{tabular}
\end{longtable}
\end{center}
The pulsars written in the bold are those for which eclipse has been reported.\\
$^{d}$: \cite{J0751_inclination};
$^{e}$: \cite{J1431_inclination_roche};
$^{g}$: \cite{J1810_inclination};
$^{h}$: \cite{J2051_0827_inclination}
%$^{i}$: \cite{J2052+1219_inclination};
$^{j}$: \cite{J1555_inclination};


 

\vspace{1cm}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
